Reconciling Event Structures with Modern Multiprocessors

Weakestmo is a recently proposed memory consistency model that uses event structures to resolve the infamous "out-of-thin-air" problem. Although it has been shown to have important benefits over other memory models, its established compilation schemes are suboptimal in that they add more fences than necessary. In this paper, we prove the correctness in Coq of the intended compilation schemes for Weakestmo to a range of hardware memory models (x86, POWER, ARMv7, ARMv8, RISC-V). Our proof is the first that establishes correctness of compilation of an event-structure-based model that forbids "thin-air" behaviors, as well as the first mechanized compilation proof of a weak memory model supporting sequentially consistent accesses to such a range of hardware platforms. Our compilation proof goes via the recent Intermediate Memory Model (IMM), which we suitably extend with sequentially consistent accesses.

==> immsc/c11.tex <==
\section{From \CC and \RC to \IMMsc}
\label{sec:c11}

In this section, we extend the correctness of the mapping from \CC and \RC models to \IMM to cover SC accesses, \ie
establish the correctness of the mapping to \IMMsc.
This extension is straightforward since \IMMsc has almost the same \ref{ax:sc} axiom as \RC.

Following \cite{Podkopaev-al:POPL19}, we consider a version of the \CC model from \cite{Batty-al:POPL11} with
fixes from~\cite{c11comp} and~\cite{Lahav-al:PLDI17}.
In this paper, we contemplate SC accesses of the model but still not the non-atomic fragment of it
since \IMMsc, like \IMM, does not have direct counterparts for non-atomic accesses.
That is, we assume the following definition of \CC-consistency.

\begin{definition}
\label{def:c11}
$G$ is called \CC-\emph{consistent} if the following hold:
\begin{itemize}
\item $\codom{G.\lRF} = G.\lR$.
\item For every location $\loc\in\Loc$, $G.\lCO$ totally orders $G.\ewlab{}{\loc}{}{}$.
\item $G.\lHBs\mathbin{;}G.\lECO^?$ is irreflexive.
\item $G.\lRMW \cap (G.\lFRE\mathbin{;}G.\lCOE) = \emptyset$.
\item $[\lF^\sco] \mathbin{;}(\lHBs \cup \lHBs\mathbin{;} \lECO\mathbin{;}\lHBs)\mathbin{;} [\lF^\sco]$ is acyclic.
\item $G.\lPSCBs \cup G.\lPSCFs$ is acyclic. \labelAxiom{sc-rc11}{ax:sccc}
\end{itemize}
\end{definition}
Here $\lPSCBs$ and $\lPSCFs$ are the same as $\lPSCB$ and $\lPSCF$ from~\cref{sec:immsc}
but defined with $\lHBs$ instead of $\lHB$ (see~\cite[Remark 2]{Podkopaev-al:POPL19}).
Since $\lHBs$ is weaker (namely, it is smaller) than $\lHB$, \CC-consistency directly follows from \IMMsc-consistency.

The \RC-consistency predicate \cite{Lahav-al:PLDI17} is defined as a strengthening of \cref{def:c11} by additionally
requiring acyclicity of $G.\lPO \cup G.\lRF$.
Since in~\cite{Podkopaev-al:POPL19} there is a proof of the correctness of a mapping from \RC to \IMM which places a (control)
dependency or a fence between every relaxed read and subsequent relaxed write
and \ref{ax:sccc} directly follows from \ref{ax:sc},
the same mapping from \RC to \IMMsc is also correct (in the presence of SC accesses).

